Logic Programming approaches for routing fault-free and maximally-parallel Wavelength Routed Optical Networks on Chip (Application paper)

One promising trend in digital system integration consists of boosting on-chip communication performance by means of silicon photonics, thus materializing the so-called Optical Networks-on-Chip (ONoCs). Among them, wavelength routing can be used to route a signal to destination by univocally associating a routing path to the wavelength of the optical carrier. Such wavelengths should be chosen so to minimize interferences among optical channels and to avoid routing faults. As a result, physical parameter selection of such networks requires the solution of complex constrained optimization problems. In previous work, published in the proceedings of the International Conference on Computer-Aided Design, we proposed and solved the problem of computing the maximum parallelism obtainable in the communication between any two endpoints while avoiding misrouting of optical signals. The underlying technology, only quickly mentioned in that paper, is Answer Set Programming (ASP). In this work, we detail the ASP approach we used to solve such problem. Another important design issue is to select the wavelengths of optical carriers such that they are spread across the available spectrum, in order to reduce the likelihood that, due to imperfections in the manufacturing process, unintended routing faults arise. We show how to address such problem in Constraint Logic Programming on Finite Domains (CLP(FD)). This paper is under consideration for possible publication on Theory and Practice of Logic Programming.

==> asp.tex <==
\section{Answer Set Programming}
\label{sec:asp}

Answer Set Programming (ASP) is a class of logic programming languages that rely on the stable model semantics \cite{StableModels},
also known as answer set semantics.
We assume a basic familiarity with logic programming and its syntax; for an introduction 
one can refer to \cite{Lloyd}.
A logic program consists of a set of rules %of the form
%
$$a \mbox{~:-~} l_1, l_2, \dots, l_n.$$
%
where $a$ is an atom (also called the {\em head} of the rule), and the $l_i$ are literals (called the {\em body} of the rule).
Rules with empty body are also called {\em facts}, while
rules with empty head are called {\em Integrity Constraints (IC)}, and their body must evaluate to {\em false}
in any model of the program.

Literals and rules containing no variables are called {\em ground}. We denote as $gr(r)$ all
possible instantiations of the rule $r$ of the program $\Pi$,
on the basis of ground facts of the program.
The {\em ground istantiation} of $\Pi$ is a program consisting of
% of all ground instances of $\Pi$,
all ground instances of rules in $\Pi$,
i.e., $gr(\Pi)=\bigcup_{r \in \Pi} gr(r)$.
For any set $M$ of atoms from $\Pi$, let $\Pi_M$ be the program obtained from $\Pi$ by deleting $(i)$ each rule that has a negative literal $\neg B$ in its body with $B\in M$ and $(ii)$ all negative literals in the bodies of the remaining rules. Since $\Pi_M$ is negation free, it has a unique minimal Herbrand model. If this model coincides with $M$, then $M$ is a Stable Model of $\Pi$ \cite{StableModels}.
In general, a program may have zero, one, or more answer sets.



Consider the following logic program $\Pi_0$ (and its grounding $gr(\Pi_0)$):
$$
\begin{array}{lllll}
\Pi_0 \left\{
\begin{array}{l}
\mbox{\tt p(1).} \\
\mbox{\tt p(2).} \\
\mbox{\tt q(X,Y):- p(X), p(Y),}\\
\qquad \mbox{\tt	X!=Y, not q(Y,X).} \\
\end{array}
\right.
\hspace{5mm}
&
gr(\Pi_0) \left\{
\begin{array}{l}
\mbox{\tt p(1).}\\
\mbox{\tt p(2).}\\
\mbox{\tt q(2,1):- not q(1,2).}\\
\mbox{\tt q(1,2):- not q(2,1).}
\end{array}
\right.
\end{array}
$$
%
The program 
$\Pi_0$ has 2 answer sets: %\code{$S_1$=\{p(1). p(2). q(1,2).\}} 
$S_1=\{p(1).~ p(2).~ q(1,2).\}$
and 
%\code{$S_2$=\{p(1). p(2). q(2,1).\}}.
$S_2=\{p(1).~ p(2).~ q(2,1).\}$.


Among the various dialects and implementations of ASP, we use the language of the grounder Gringo \cite{Gringo},
that extends the basic logic programming syntax with a number of features.
We show the most relevant to this article, while the interested reader can refer to  \cite{Gringo} for a complete description.

\paragraph{Intervals}
If an atom $a(i..j)$, where $i$ and $j$ are integers, is in a clause, the clause is repeated for all possible values $k$ such that $i\leq k \leq j$.
For example, the fact $a(1..4).$ is expanded to four facts, namely 
%\begin{lstlisting}
\code {a(1). a(2). a(3). a(4).}
%\end{lstlisting}

\paragraph{Conditions} allow for instantiating variables to collections of terms within a single rule.
A condition has the syntax $a(X):c(X)$, and it is expanded to as many $a(X)$ atoms as those making true the atom $c(X)$.
For example, consider the program $\Pi_1$ and its grounding $gr(\Pi_1)$
$$\begin{array}{llll}
\Pi_1 \left\{
	\begin{array}{l}
		\mbox{\tt p(1..3).} \\
		\mbox{\tt q:- r(X):p(X).} 
	\end{array}
	\right.
	& \qquad &
gr(\Pi_1) \left\{
	\begin{array}{l}
		\mbox{\tt p(1). p(2). p(3).} \\
		\mbox{\tt q:- r(1), r(2), r(3).}
	\end{array}
	\right.
\end{array}
$$

\noindent Notice that the condition in the body is expanded to a conjunction.%, while the condition in the head of the rule is expanded as a disjunction.

\paragraph{Counting} \cite{WeightConstraints}
If $a_1,a_2,a_3,\dots$ are atoms, and $l$ and $u$ are integers,
the aggregate
$$l \ \{ a_1, a_2, a_3, \dots \} \ u$$
is true for every set S of atoms including from l to u members of $\{ a_1, a_2, a_3, \dots \}$,
i.e., $l \leq | \{ a_i \in S \} | \leq u$. Trivial bounds can be omitted.

\paragraph{Summation}
If $a_1, a_2, a_3, \dots$ are atoms and $v_1, v_2, v_3,\dots$ are integers, the
aggregate
$$l \ {\bf\sharp sum} [ a_1 = v_1, a_2 = v_2, a_3 = v_3, \dots ] \ u$$
is true for every set S of atoms such that the sum of $v_i$ over included members
$a_i$ of $\{ a_1, a_2, a_3, \dots \}$ is in the interval $[l,u]$:
$$l \leq \sum_{i:a_i\in S} v_i \leq u$$

\subsubsection{ASP solvers.}
Usually, ASP solvers \cite{WeightConstraints,ASSAT,Cmodels,DLV_ToCL,potassco} work in two stages.
In the first, called {\em grounding}, the program is converted into an equivalent ground program. %The ground program is always finite due to the syntactic restrictions on the input language.
The ground program can be very large, % (possibly, exponential in the size of the original program),
depending on the input program.
The second stage is devoted to looking for stable models (answer sets) of the ground program.
